Cross-Modal Binary Attention: An Energy-Efficient Fusion Framework for Audio-Visual Learning

Effective multimodal fusion requires mechanisms that can capture complex cross-modal dependencies while remaining computationally scalable for real-world deployment. Existing audio-visual fusion approaches face a fundamental trade-off: attention-based methods effectively model cross-modal relationships but incur quadratic computational complexity that prevents hierarchical, multi-scale architectures, while efficient fusion strategies rely on simplistic concatenation that fails to extract complementary cross-modal information. We introduce CMQKA, a novel cross-modal fusion mechanism that achieves linear O(N) complexity through efficient binary operations, enabling scalable hierarchical fusion previously infeasible with conventional attention. CMQKA employs bidirectional cross-modal Query-Key attention to extract complementary spatiotemporal features and uses learnable residual fusion to preserve modality-specific characteristics while enriching representations with cross-modal information. Building upon CMQKA, we present SNNergy, an energy-efficient multimodal fusion framework with a hierarchical architecture that processes inputs through progressively decreasing spatial resolutions and increasing semantic abstraction. This multi-scale fusion capability allows the framework to capture both local patterns and global context across modalities. Implemented with event-driven binary spike operations, SNNergy achieves remarkable energy efficiency while maintaining fusion effectiveness and establishing new state-of-the-art results on challenging audio-visual benchmarks, including CREMA-D, AVE, and UrbanSound8K-AV, significantly outperforming existing multimodal fusion baselines. Our framework advances multimodal fusion by introducing a scalable fusion mechanism that enables hierarchical cross-modal integration with practical energy efficiency for real-world audio-visual intelligence systems.

==> 01_introduction_section.tex <==
\section{Introduction}

Multimodal learning has emerged as a fundamental research direction in artificial intelligence, enabling systems to process and integrate information from multiple sensory modalities such as vision, audio, and text~\cite{baltrusaitis_2019_multimodal_machine_learning, ramachandram_2017_deep_multimodal_learning}. By replicating the human ability to integrate complementary information across modalities, multimodal systems create robust representations that surpass unimodal approaches~\cite{yuille_2006_vision_as_bayesian}. Audio-visual learning, in particular, has demonstrated significant benefits across diverse tasks including speech recognition~\cite{afouras_2018_deep_audio_visual}, emotion recognition~\cite{barros_2016_developing_crossmodal_expression}, event localization~\cite{tian_2018_audio_visual_event_localization}, and action recognition~\cite{kazakos_2019_epic_fusion_audio}. However, effective multimodal fusion faces fundamental challenges including inherent differences in feature distributions across modalities, varying information quality, and the potential for modality conflicts during integration~\cite{wang_2020_what_makes_training, pham_2019_found_in_translation}.

The success of attention mechanisms in capturing long-range dependencies has naturally led to their adoption for cross-modal fusion~\cite{long_2022_multimodal_attentive_fusion, moorthy_2025_hybrid_multi_attention_network}. Cross-modal attention enables models to selectively focus on relevant features from one modality while processing another, facilitating deep feature interaction and learning of complex cross-modal correlations. However, conventional attention mechanisms suffer from a critical limitation: quadratic computational and memory complexity with respect to the number of tokens or spatial locations. For instance, standard self-attention as used in transformers~\cite{vaswani_2017_attention_is_all} requires $O(N^2)$ operations, where $N$ represents the sequence length. This quadratic scaling creates a fundamental trade-off between fusion effectiveness and computational scalability, severely limiting the construction of hierarchical, multi-scale architectures essential for capturing both local and global patterns in multimodal data~\cite{zhou_2022_spikformer_when_spiking_neural}.

Recent work has explored linear-complexity alternatives to address this scalability barrier. In the domain of efficient neural architectures, Query-Key attention mechanisms have demonstrated the possibility of achieving linear $O(N)$ complexity through simplified attention computation~\cite{zhou_2024_qkformer_hierarchical_spiking}. However, these approaches have been primarily developed for unimodal scenarios and do not directly address cross-modal fusion challenges. Conversely, multimodal fusion methods that do employ cross-modal attention, such as \ac{SCMRL}~\cite{he_2025_enhancing_audio_visual}, rely on conventional quadratic-complexity attention mechanisms. \ac{SCMRL} introduces \ac{CCSSA} to extract complementary audio-visual features through cross-modal attention, incorporating these features as residuals to preserve modality-specific characteristics. While effective for single-scale fusion, the quadratic complexity of \ac{CCSSA} prevents the construction of deep hierarchical architectures with multiple fusion stages at varying spatial resolutions.

This computational barrier has profound implications for multimodal fusion systems. Hierarchical multi-scale processing, which progressively decreases spatial resolution while increasing semantic abstraction across network stages, has proven essential for robust visual recognition~\cite{he_2016_deep_residual_learning} and has recently been extended to efficient unimodal architectures~\cite{zhou_2024_qkformer_hierarchical_spiking}. However, applying this architectural principle to multimodal fusion requires cross-modal attention at each hierarchical stage, multiplying the computational cost and making it prohibitive for real-world deployment. The field thus lacks a cross-modal attention mechanism that combines the effectiveness of attention-based fusion with the linear computational complexity necessary for hierarchical multi-scale processing.

To address these challenges, we introduce \ac{CMQKA}, a novel cross-modal attention mechanism that achieves linear $O(N)$ complexity while enabling effective extraction of complementary spatiotemporal features across modalities. \ac{CMQKA} extends the Query-Key attention paradigm to the cross-modal domain, employing bidirectional attention where queries from one modality attend to keys from another modality using efficient binary operations. Through learnable residual fusion, \ac{CMQKA} preserves modality-specific characteristics while enriching representations with complementary cross-modal information. The linear complexity of \ac{CMQKA} enables the construction of hierarchical multimodal architectures with multiple fusion stages, each operating at progressively coarser spatial scales and higher semantic levels. We implement this mechanism within SNNergy, an energy-efficient multimodal fusion framework that leverages event-driven binary spike operations to further reduce computational overhead while maintaining fusion effectiveness. Our framework processes audio-visual inputs through a three-stage hierarchical architecture, achieving both superior recognition performance and remarkable efficiency compared to existing fusion approaches. Our main contributions are as follows.
\begin{itemize}
    \item We propose \ac{CMQKA}, a novel cross-modal attention mechanism that achieves linear $O(N)$ computational complexity while effectively extracting complementary spatiotemporal features across audio and visual modalities. Through bidirectional Query-Key attention and learnable residual fusion, \ac{CMQKA} enables deep cross-modal feature interaction while preserving modality-specific characteristics, addressing the scalability limitations of conventional quadratic-complexity cross-modal attention.

    \item We present SNNergy, an energy-efficient hierarchical multimodal fusion framework that leverages \ac{CMQKA} to enable multi-scale cross-modal integration across three hierarchical stages with progressively decreasing spatial resolutions and increasing semantic abstraction. By implementing fusion through event-driven binary operations, SNNergy achieves practical computational efficiency for real-world audio-visual intelligence systems.

    \item We demonstrate through extensive experiments on challenging audio-visual benchmarks (UrbanSound8K-AV, AVE,CREMA-D) that our fusion approach establishes new state-of-the-art results, significantly outperforming existing multimodal fusion methods in both classification accuracy and computational efficiency, validating the effectiveness of linear-complexity hierarchical cross-modal attention for scalable multimodal intelligence.
\end{itemize}


% The remainder of this paper is organized as follows. Section~2 reviews related work on spiking neural networks, multimodal learning, and attention mechanisms. Section~3 presents the SNNergy architecture in detail, including the hierarchical framework, \ac{CMQKA} mechanism, and residual fusion strategy. Section~4 describes our experimental setup, datasets, and implementation details. Section~5 presents comprehensive results including performance comparisons, ablation studies, and robustness analysis under various conditions. Section~6 discusses the implications of our findings, limitations of the current approach, and promising directions for future research. Finally, Section~7 concludes the paper with a summary of our contributions and their broader impact on the field of neuromorphic computing and multimodal learning.


==> 02_related_work_section.tex <==
\section{Related Work}

Two mainstream approaches exist for obtaining trained \ac{SNN}s: \ac{ANN}-to-\ac{SNN} conversion and direct training methods. The conversion approach transforms pre-trained \ac{ANN}s into \ac{SNN}s by replacing activation functions with spiking neurons \cite{cao_2015_spiking_deep_convolutional, rueckauer_2017_conversion_of_continuous}. While this method leverages well-established \ac{ANN} architectures, it often suffers from performance degradation and requires long inference latencies with numerous time steps \cite{bu_2023_optimal_ann_snn_conversion}.

Direct training of \ac{SNN}s has gained substantial attention as a more effective alternative. The primary challenge in direct training lies in the non-differentiable nature of spike generation, which prevents the direct application of standard backpropagation. To address this, surrogate gradient methods have been developed, where smooth surrogate functions approximate the discontinuous spike activation during the backward pass \cite{neftci_2019_surrogate_gradient_learning, wu_2018_spatio_temporal_backpropagation}. \ac{BPTT} combined with surrogate gradients forms the foundation of modern \ac{SNN} training \cite{zenke_2018_superspike_supervised_learning}. \ac{STBP} extends \ac{BPTT} by considering gradient updates in both spatial and temporal domains \cite{wu_2018_spatio_temporal_backpropagation}. Recent advances have introduced more efficient training algorithms such as \ac{OTTT} and \ac{SLTT} to reduce memory consumption during training \cite{chang_2024_direct_training_high}. Various refinements to surrogate gradient methods, including learnable surrogate gradients and masked surrogate gradients, have further improved training stability and model generalization \cite{lian_2023_learnable_surrogate_gradient, chen_2024_directly_training_temporal}.

The integration of the Transformer architecture with \ac{SNN}s has opened new avenues for achieving both high performance and energy efficiency. Spikformer, introduced by \cite{zhou_2022_spikformer_when_spiking_neural}, pioneered this direction by proposing \ac{SSA}, which models sparse visual features using spike-form Query, Key, and Value representations without requiring softmax operations. By leveraging the binary nature of spikes, \ac{SSA} replaces expensive multiplication operations with simple masking and addition, achieving significant energy savings while maintaining competitive performance on both static and neuromorphic datasets \cite{zhou_2022_spikformer_when_spiking_neural}.

Building upon Spikformer, several variants have been developed to further enhance performance and efficiency. Spikingformer introduced spike-driven residual structures that reduce non-spiking computations by reordering the placement of neuron layers \cite{zhou_2023_spikingformer_spike_driven}. The Spike-Driven Transformer proposed the \ac{SDSA} mechanism, which utilizes only masking and addition operations to eliminate multiplication entirely \cite{yao_2023_spike_driven_transformer}. Recent work on Spiking Transformers with spatial-temporal attention has demonstrated the importance of capturing both spatial and temporal dependencies in spike-based processing, addressing limitations of spatial-only attention mechanisms \cite{lee_2025_spiking_transformer_with}.

Despite these advances, the quadratic computational complexity of \ac{SSA} with respect to the number of tokens poses challenges for constructing hierarchical architectures with multi-scale representations. QKFormer addresses this limitation by introducing a novel Q-K attention mechanism with linear complexity \cite{zhou_2024_qkformer_hierarchical_spiking}. Unlike \ac{SSA}, which requires Query, Key, and Value components, Q-K attention uses only Query and Key to compute attention weights through binary spike vectors. Specifically, \ac{QKTA} computes row-wise summation over the Key matrix to generate a token attention vector, which is then used to mask the Key matrix for selective feature aggregation. Similarly, \ac{QKCA} performs column-wise summation for channel-wise attention. The linear complexity of Q-K attention enables QKFormer to construct hierarchical architectures with decreasing token numbers across stages, achieving multi-scale spiking representations. Furthermore, QKFormer introduces the \ac{SPEDS} module, which enhances spiking information transmission across downsampling blocks through residual learning. With these innovations, QKFormer achieved groundbreaking results, becoming the first directly-trained \ac{SNN} to exceed 85\% top-1 accuracy on ImageNet-1K \cite{zhou_2024_qkformer_hierarchical_spiking}.

Multimodal learning, particularly audio-visual integration, has demonstrated significant advantages over unimodal approaches by leveraging complementary information from multiple sensory modalities. Human perception naturally integrates visual and auditory cues to understand the environment, and replicating this capability in artificial systems has been a longstanding goal in machine learning \cite{baltrusaitis_2019_multimodal_machine_learning}. The fundamental challenge in multimodal fusion lies in effectively extracting and integrating complementary cross-modal features while managing the computational complexity and energy demands of such systems.

Various fusion strategies have been explored to address these challenges. Early fusion combines features from different modalities at the input level, enabling the model to learn joint representations from the outset \cite{ramachandram_2017_deep_multimodal_learning}. Late fusion processes each modality independently through separate networks and combines their outputs at the decision level \cite{gadzicki_2020_early_vs_late}. Intermediate fusion, also known as hybrid fusion, integrates features at multiple stages of the network, balancing the benefits of both early and late fusion \cite{liu_2024_multimodal_alignment_and}. While these classical approaches provide different trade-offs between integration depth and computational overhead, they often rely on simple concatenation or weighted averaging, failing to adequately model the complex inter-modal dependencies present in audio-visual data.

Attention-based fusion mechanisms have emerged as a promising direction, offering the ability to dynamically weight modality contributions and capture cross-modal relationships \cite{long_2022_multimodal_attentive_fusion, moorthy_2025_hybrid_multi_attention_network}. Cross-modal attention enables information from one modality to guide the feature extraction of another, establishing fine-grained correspondences between audio and visual events \cite{arandjelovic_2018_objects_that_sound}. Cross-modal distillation transfers knowledge from a strong modality to a weaker one, improving overall performance \cite{gupta_2022_cross_modal_distillation}. However, traditional attention mechanisms based on scaled dot-product attention suffer from quadratic computational complexity with respect to sequence length, making them prohibitively expensive for high-resolution multimodal inputs or resource-constrained deployment scenarios.

Beyond computational complexity, several critical challenges persist in audio-visual fusion. Temporal alignment remains difficult, as audio and visual signals may have different temporal resolutions and sampling rates \cite{arandjelovic_2017_look_listen_and}. Modality imbalance, where one modality provides more discriminative information than the other, can lead to suboptimal fusion if not properly addressed \cite{wang_2020_what_makes_training}. Additionally, noise and signal variability in real-world scenarios pose challenges for robust multimodal recognition \cite{hu_2018_squeeze_and_excitation}. Crucially, the energy consumption of deep multimodal fusion systems limits their deployment on edge devices and mobile platforms, where battery life and thermal constraints are paramount. This has motivated research into energy-efficient fusion architectures that maintain accuracy while reducing computational overhead.

Addressing the energy efficiency challenge in multimodal fusion requires fundamentally rethinking the computational substrate. Event-driven computing paradigms, particularly \acp{SNN}, offer a promising path forward by replacing dense floating-point operations with sparse, binary spike events that trigger computation only when necessary \cite{maass_1997_networks_of_spiking}. This event-driven nature enables dramatic energy savings: neuromorphic hardware implementations of spiking networks can achieve orders-of-magnitude lower power consumption compared to conventional GPU-based inference \cite{davies_2018_loihi_a_neuromorphic}. However, translating effective multimodal fusion mechanisms to the spiking domain while preserving both fusion quality and computational efficiency remains an open challenge. Early attempts at audio-visual fusion in spiking networks relied on simple concatenation strategies \cite{kim_2021_audio_visual_spiking} that failed to capture cross-modal complementarity, highlighting the need for specialized attention-based fusion mechanisms adapted to spike-based computation.

Recent work has made progress in developing cross-modal attention mechanisms for energy-efficient fusion. The \ac{SCMRL} framework \cite{he_2025_enhancing_audio_visual} introduces the \ac{CCSSA} mechanism for extracting complementary audio-visual features through spatiotemporal cross-modal attention. \ac{CCSSA} decomposes cross-modal fusion into spatial and temporal pathways: the \ac{SCSA} component computes cross-modal attention across spatial dimensions by using Query from one modality and Key-Value from another, while \ac{TCSA} captures temporal complementarity along the time dimension. These complementary features are combined through element-wise multiplication and integrated as residuals into the original modality-specific representations, preserving unimodal discriminative power while enriching features with cross-modal information. Additionally, \ac{SCMRL} employs a \ac{SAO} mechanism using contrastive learning to align cross-modal features in a shared semantic space, addressing distributional shifts between modalities. This fusion approach achieves strong performance on audio-visual benchmarks (CREMA-D, UrbanSound8K-AV) while leveraging event-driven spiking computation for energy efficiency \cite{he_2025_enhancing_audio_visual}.

However, a critical limitation constrains SCMRL's fusion architecture: the \ac{CCSSA} mechanism relies on conventional spiking self-attention with quadratic $O(N^2)$ computational complexity, where $N$ is the number of spatial tokens. This quadratic scaling fundamentally prevents the construction of hierarchical multi-scale fusion architectures, as the computational cost of cross-modal attention at multiple resolutions becomes prohibitive. Consequently, SCMRL is restricted to single-scale, non-hierarchical fusion, limiting its ability to capture audio-visual correspondences across multiple spatial and temporal scales—a capability proven essential in state-of-the-art vision architectures \cite{liu_2021_swin_transformer_hierarchical}. This reveals a critical gap in existing energy-efficient multimodal fusion approaches: the lack of a cross-modal attention mechanism that combines linear computational complexity with effective complementary feature extraction, enabling scalable hierarchical fusion previously infeasible in resource-constrained deployments.

Recent work has further advanced multimodal \ac{SNN} architectures through innovations in neuron-level fusion and temporal attention mechanisms. MISNet \cite{liu_2025_towards_energy_efficient} introduces the Multimodal Leaky Integrate-and-Fire (MLIF) neuron, which coordinates spike activations from audio and visual modalities within a single neuron rather than through separate processing pathways. This neuron-level integration enables synchronized spike emissions across modalities, addressing the cross-modal asynchronization issue that arises from heterogeneous distributions in audio-visual data. Through multi-round spike interaction and modality-specific loss regularization, MISNet demonstrates improved balance between accuracy and energy efficiency on audio-visual classification tasks. Complementing this neuron-level innovation, recent work on temporal attention-guided adaptive fusion \cite{shen_2025_spiking_neural_networks} addresses modality imbalance by dynamically assigning importance scores to fused features at each timestep. This approach enables hierarchical integration of temporally heterogeneous spike-based features while modulating learning rates per modality based on attention scores, preventing dominant modalities from monopolizing optimization. These advances underscore the critical role of both neuron-level mechanisms and temporal dynamics in achieving balanced, efficient multimodal learning in \ac{SNN}s.

To address the critical gap in scalable, energy-efficient multimodal fusion, we propose SNNergy, a hierarchical audio-visual fusion framework that introduces \ac{CMQKA}—the first cross-modal attention mechanism achieving linear $O(N)$ computational complexity while preserving effective complementary feature extraction. SNNergy builds upon complementary insights from prior work: QKFormer demonstrates that linear-complexity Query-Key attention enables hierarchical multi-scale architectures infeasible with quadratic attention \cite{zhou_2024_qkformer_hierarchical_spiking}, while SCMRL establishes that residual integration of cross-modal complementary features preserves modality-specific discriminative power \cite{he_2025_enhancing_audio_visual}. However, both approaches address orthogonal challenges—QKFormer targets unimodal hierarchical processing, while SCMRL achieves cross-modal fusion with non-hierarchical, quadratic-complexity attention. SNNergy synergizes these complementary strengths to enable scalable hierarchical multimodal fusion.

Our framework advances multimodal fusion through three key innovations addressing the scalability-effectiveness trade-off. First, we introduce \ac{CMQKA}, extending the Query-Key attention paradigm to cross-modal fusion with linear $O(N)$ complexity. Unlike SCMRL's \ac{CCSSA} mechanism (quadratic $O(N^2)$ complexity), \ac{CMQKA} computes channel-aggregated attention vectors rather than full token-to-token attention matrices, enabling efficient cross-modal feature interaction without sacrificing complementary information extraction. This linear complexity fundamentally enables hierarchical fusion architectures previously computationally infeasible. Second, we demonstrate the first hierarchical multi-scale cross-modal fusion framework in energy-efficient computing, processing audio-visual inputs through three progressively coarser spatial resolutions with cross-modal attention at each scale. This hierarchical design captures audio-visual correspondences across multiple spatial and temporal granularities—a capability absent in SCMRL's single-scale architecture—proving crucial for robust multimodal recognition. Third, we propose bidirectional symmetric cross-modal attention ensuring balanced information flow: both audio and visual pathways equally benefit from cross-modal complementarity through symmetric Query-Key projections, preventing asymmetric modality dominance.

Implemented using event-driven spiking computation, SNNergy achieves both fusion scalability and energy efficiency. By leveraging sparse binary spike operations throughout the hierarchical architecture, our framework maintains the low-power advantages of neuromorphic processing while delivering superior multimodal fusion performance. Extensive experiments validate that linear-complexity cross-modal attention, hierarchical multi-scale fusion, and energy-efficient implementation collectively enable practical deployment of sophisticated audio-visual intelligence in resource-constrained environments.


==> 03_preliminary_section.tex <==
\section{Preliminary}
In this section, we introduce the problem defination for the audio-video problem. Then we provide a brief overview of the fundamental components that for our proposed SNNergy framework, including the \ac{LIF} neuron model,  and the Query-Key attention mechanism adapted multimodality.
\subsection{Problem Definition}

Consider a multimodal learning task where the objective is to learn a mapping from paired audio-visual inputs to a set of semantic labels. Let $\mathcal{D} = \{(\mathbf{X}_i^a, \mathbf{X}_i^v, y_i)\}_{i=1}^{N}$ denote the training dataset consisting of $N$ samples, where $\mathbf{X}_i^a \in \mathbb{R}^{T_a \times F_a}$ represents the audio input with $T_a$ temporal frames and $F_a$ frequency bins (e.g., mel-spectrogram features), $\mathbf{X}_i^v \in \mathbb{R}^{T_v \times H \times W \times 3}$ represents the visual input comprising $T_v$ frames of height $H$ and width $W$ with RGB channels, and $y_i \in \{1, 2, \ldots, C\}$ denotes the ground-truth label from $C$ semantic categories.

The primary objective is to learn a multimodal function $f_{\theta}: \mathcal{X}^a \times \mathcal{X}^v \rightarrow \mathcal{Y}$ parameterized by $\theta$, which maps the joint audio-visual input space $\mathcal{X}^a \times \mathcal{X}^v$ to the label space $\mathcal{Y} = \{1, \ldots, C\}$. Formally, the learning problem can be expressed as:
\begin{equation}
    \theta^* = \arg\min_{\theta} \sum_{i=1}^{N} \mathcal{L}(f_{\theta}(\mathbf{X}_i^a, \mathbf{X}_i^v), y_i) + \lambda \Omega(\theta),
\end{equation}
where $\mathcal{L}(\cdot, \cdot)$ is a loss function (e.g., cross-entropy loss for classification tasks), $\Omega(\theta)$ represents a regularization term, and $\lambda$ controls the regularization strength.

In this study, we focus on designing the multimodal function $f_{\theta}$ using spiking neural network architectures that effectively integrate audio and visual information while leveraging the temporal dynamics inherent in spike-based processing. The proposed SNNergy framework aims to address the challenges of cross-modal fusion, and efficient representation learning within the spiking domain.

\subsection{\ac{LIF} Neuron Model}

The \ac{LIF} neuron serves as the fundamental computational in \acp{SNN}, providing biologically-plausible temporal dynamics for spike-based information processing. At each time step $t$, the membrane potential $V_i^t$ of the $i$-th neuron evolves according to the discrete-time leaky integration dynamics:
\begin{equation}
    V_i^t = \tau V_i^{t-1}(1 - S_i^{t-1}) + W_i X_i^t,
\end{equation}
where $\tau \in (0, 1)$ is the membrane decay constant controlling the leakage rate, $S_i^{t-1} \in \{0, 1\}$ is the binary spike output from the previous time step, $W_i$ represents the synaptic weights, and $X_i^t$ denotes the input current at time $t$. The neuron generates a spike when the membrane potential exceeds a threshold $V_{\text{th}}$, implemented through the Heaviside step function:
\begin{equation}
    S_i^t = H(V_i^t - V_{\text{th}}) = \begin{cases}
        1, & \text{if } V_i^t \geq V_{\text{th}}, \\
        0, & \text{otherwise}.
    \end{cases}
\end{equation}
Following spike emission, the membrane potential undergoes a hard reset as indicated by the $(1 - S_i^{t-1})$ term in the dynamics equation. During backpropagation, the non-differentiable Heaviside function is approximated using a surrogate gradient function to enable gradient-based training~\cite{neftci_2019_surrogate_gradient_learning, wu_2018_spatio_temporal_backpropagation}.

\subsection{Self Attention in Spiking Neural Networks}

The transformer architecture relies fundamentally on the self-attention mechanism to capture long-range dependencies and model complex relationships within input sequences. In the vanilla self-attention mechanism~\cite{vaswani_2017_attention_is_all}, three floating-point components—Query ($\mathbf{Q}_F$), Key ($\mathbf{K}_F$), and Value ($\mathbf{V}_F$)—are derived from the input $\mathbf{X0}$ through learnable linear projections: $\mathbf{Q}_F, \mathbf{K}_F, \mathbf{V}_F = \mathbf{X}(\mathbf{W}_Q, \mathbf{W}_K, \mathbf{W}_V)$. The attention output is computed as:
\begin{equation}
    \text{VSA}(\mathbf{Q}_F, \mathbf{K}_F, \mathbf{V}_F) = \text{Softmax}\left(\frac{\mathbf{Q}_F\mathbf{K}_F^T}{\sqrt{d}}\right)\mathbf{V}_F,
\end{equation}
where $d$ is the dimension of the key vectors and the scaling factor $1/\sqrt{d}$ normalizes the attention scores. However, this formulation presents significant challenges for \acp{SNN}: the softmax operation involves exponential calculations and division, while the matrix multiplications operate on continuous floating-point values both of which are incompatible with the discrete, event-driven nature of spike-based computation.

To address these incompatibilities, \ac{SSA}~\cite{zhou_2022_spikformer_when_spiking_neural} reformulates the attention mechanism to operate entirely with binary spike representations. The spike-form Query, Key, and Value matrices are generated through learnable linear layers followed by batch normalization and spiking neurons: $\mathbf{I} = \text{SN}_I(\text{BN}_I(\mathbf{X}\mathbf{W}_I))$ for $\mathbf{I} \in \{\mathbf{Q}, \mathbf{K}, \mathbf{V}\}$, where $\mathbf{Q}, \mathbf{K}, \mathbf{V} \in \{0, 1\}^{T \times N \times D}$. The \ac{SSA} computation is then formulated as:
\begin{equation}
    \text{SSA}(\mathbf{Q}, \mathbf{K}, \mathbf{V}) = \text{SN}\left(\mathbf{Q}\mathbf{K}^T\mathbf{V} \times s\right),
\end{equation}
where $s$ is a learnable scaling factor and SN denotes the spiking neuron layer. By replacing continuous multiplications with sparse binary operations and eliminating the softmax function, \ac{SSA} achieves substantial energy efficiency while preserving the core attention mechanism. However, the computational complexity of \ac{SSA} remains $O(N^2D)$, scaling quadratically with the number of tokens $N$, which severely constrains the construction of hierarchical architectures with multi-scale feature representations.

\subsection{Query-Key Linear Attention}

To overcome the quadratic complexity bottleneck of \ac{SSA}~\cite{zhou_2022_spikformer_when_spiking_neural} that restricts hierarchical spiking transformer architectures, we adopt the Query-Key attention mechanism~\cite{zhou_2024_qkformer_hierarchical_spiking}, which achieves linear computational complexity while operating exclusively with binary spike operations. Given spike-form input $\mathbf{X} \in \{0, 1\}^{T \times N \times D}$, the Query ($\mathbf{Q}$) and Key ($\mathbf{K}$) matrices are generated through learnable linear transformations followed by batch normalization and \ac{LIF} neurons: $\mathbf{Q} = \text{SN}_Q(\text{BN}(\mathbf{X}\mathbf{W}_Q))$ and $\mathbf{K} = \text{SN}_K(\text{BN}(\mathbf{X}\mathbf{W}_K))$, where $\mathbf{Q}, \mathbf{K} \in \{0, 1\}^{T \times N \times D}$ with $N$ tokens and $D$ channels. In the \ac{QKTA} variant, a token attention vector $\mathbf{A}_t \in \{0, 1\}^{N \times 1}$ is computed by row-wise summation over the channel dimension followed by a spiking neuron: $\mathbf{A}_t = \text{SN}(\sum_{i=0}^{D} \mathbf{Q}_{i,j})$, which models the binary importance of different tokens. The output is then obtained through a column-wise mask operation (Hadamard product): $\mathbf{X}' = \mathbf{A}_t \otimes \mathbf{K}$, followed by a post-linear layer $\mathbf{X}'' = \text{SN}(\text{BN}(\text{Linear}(\mathbf{X}')))$. This mechanism achieves $O(N)$ or $O(D)$ complexity depending on the attention dimension~\cite{zhou_2024_qkformer_hierarchical_spiking}, enabling the construction of hierarchical architectures with progressively decreasing spatial resolution across stages. The mask operation can be implemented on neuromorphic hardware, maintaining the energy-efficient properties of spike-based computation.


==> 04_methods_section.tex <==
\section{Methods}
\subsection{Cross-Modal Query-Key Attention}

A fundamental challenge in multimodal spiking neural networks is enabling efficient interaction between modalities without experiencing the quadratic computational cost that limits architectural depth. Existing cross-modal attention mechanisms~\cite{he_2025_enhancing_audio_visual} operate on the $O(N^2)$ complexity paradigm, restricting their use to single-scale, non-hierarchical designs. To overcome this limitation, we introduce the \ac{CMQKA} module, which extends the linear-complexity Q-K attention mechanism to the multimodal domain.

Our key insight is that cross-modal complementarity can be captured through Query-Key projections: one modality provides the Query that encodes "what information to seek," while the other modality provides the Key representing "what information is available." By decomposing attention into separate spatial and temporal attentions, and leveraging binary spike operations throughout, \ac{CMQKA} achieves $O(N)$ complexity while extracting rich complementary spatiotemporal features between audio and visual modalities. These cross-modal features are then integrated with the original modality-specific representations through learnable residual connections, preserving modality-specific power while enriching representations with complementary information. For clarity, we present the mechanism for a single sample with single-head attention; multi-head extensions follow standard practice.

\subsubsection*{Complementary Spatial Attention}

\begin{figure}[th]
    \centering
    \includegraphics[width=\textwidth]{imgs/qk_spatial_attention.pdf}
    \caption{Illustration of the Complementary Spatial Attention pathway within the \ac{CMQKA} module. Video spikes $\mathbf{V}' \in \{0,1\}^{T \times B \times C \times N}$ and audio spikes $\mathbf{A}' \in \{0,1\}^{T \times B \times C \times N}$ are transformed through learnable projections to generate Query $\mathbf{Q}_v$ and Key $\mathbf{K}_a$, both in $\{0,1\}^{T \times B \times C \times N}$. For multi-head attention, Q is reshaped to $\{0,1\}^{T \times B \times h \times C_h \times N}$ where $h$ is the number of heads and $C_h = C/h$ is the per-head channel dimension. The Query is summed over the per-head channel dimension $C_h$ and passed through a spiking neuron (SN) to produce binary spatial attention tensor $\mathbf{A}^{(s)} \in \{0,1\}^{T \times B \times h \times 1 \times N}$. This attention tensor selectively masks the Key matrix through element-wise multiplication ($\mathbf{S}^{v \leftarrow a} = \mathbf{A}_t^{(s)} \odot \mathbf{K}_a$) to extract complementary spatial features from the audio modality that are relevant to the video modality. The mechanism maintains $O(N)$ linear complexity through binary spike operations, avoiding the quadratic cost of traditional self-attention.}
    \label{fig:complementary_spatial_attention}
\end{figure}

Spatial correspondence between audio and visual modalities is fundamental to audio-visual scene understanding. However, determining which spatial regions in one modality complement features in another requires selective attention mechanisms. Our Complementary Spatial Attention pathway addresses this challenge by operating on the token dimension to identify and extract spatially-aligned cross-modal features, as illustrated in \cref{fig:complementary_spatial_attention}.

Given spike-form video and audio inputs $\mathbf{V}, \mathbf{A} \in \{0, 1\}^{T \times C \times H \times W}$, we flatten the spatial dimensions to obtain $\mathbf{V}', \mathbf{A}' \in \{0, 1\}^{T \times C \times N}$ with $N = H \times W$ tokens. To enable cross-modal spatial attention, we employ asymmetric projections: Query derives from the video modality to encode spatial patterns of interest, while Key derives from the audio modality to represent available auditory information. Both are generated through modality-specific learnable transformations:
\begin{equation}
    \mathbf{Q}_v = \text{SN}_Q(\text{BN}(\text{Conv1D}(\mathbf{V}', \mathbf{W}_Q^v))), \quad \mathbf{K}_a = \text{SN}_K(\text{BN}(\text{Conv1D}(\mathbf{A}', \mathbf{W}_K^a))),
\end{equation}
where $\mathbf{Q}_v, \mathbf{K}_a \in \{0, 1\}^{T \times C \times N}$. This asymmetric design enables the network to learn which audio tokens are spatially relevant to specific visual content.

To achieve linear complexity, we compute a binary spatial attention mask by aggregating the Query matrix over channels.
\begin{equation}
    \mathbf{A}_t^{(s)} = \text{SN}\left(\sum_{c=1}^{C} \mathbf{Q}_{v}[t, c, :]\right), \quad \mathbf{A}_t^{(s)} \in \{0, 1\}^{T \times 1 \times N},
\end{equation}
where the channel-wise summation captures the overall importance of each spatial token, and the spiking neuron converts accumulated membrane potentials into binary attention weights. This attention vector identifies which audio tokens are complementary to the video modality at each timestep. We then extract complementary spatial features through selective masking:
\begin{equation}
    \mathbf{S}^{v \leftarrow a} = \mathbf{A}_t^{(s)} \odot \mathbf{K}_a,
\end{equation}
where the Hadamard product $\odot$ (with broadcasting) retains only those audio tokens deemed relevant by the video-derived attention mask, yielding $\mathbf{S}^{v \leftarrow a} \in \{0, 1\}^{T \times C \times N}$. To enhance representational capacity, we refine these features through a spiking \ac{MLP} with residual connection:
\begin{equation}
    \mathbf{S}_{\text{out}}^{v \leftarrow a} = \mathbf{S}^{v \leftarrow a} + \text{MLP}(\mathbf{S}^{v \leftarrow a}),
\end{equation}
maintaining spike-form processing throughout while enabling nonlinear feature transformation.
\subsubsection*{Complementary Temporal Attention}
\begin{figure}[th]
    \centering
    \includegraphics[width=\textwidth]{imgs/qk_temporal_attention.pdf}
    \caption{Illustration of the Complementary Temporal Attention pathway within the \ac{CMQKA} module. The spatially-flattened inputs $\mathbf{V}', \mathbf{A}' \in \{0,1\}^{T \times C \times N}$ are first permuted to $N \times C \times T$ to operate along the temporal dimension. The permuted inputs are transformed through learnable projections to generate Query $\mathbf{Q}_v$ from video and Key $\mathbf{K}_a$ from audio, both in $\{0,1\}^{N \times C \times T}$ and then permuted back to $T \times C \times N$. The Query matrix is summed over channels and passed through a spiking neuron to produce binary temporal attention vector $\mathbf{A}^{(t)} \in \{0,1\}^{T \times 1 \times N}$. This attention vector selectively masks the Key matrix through element-wise multiplication ($\mathbf{T}^{v \leftarrow a} = \mathbf{A}_t^{(t)} \odot \mathbf{K}_a^{(t)}$) to extract complementary temporal features $\mathbf{T}^{v \leftarrow a}$ from the audio modality that capture temporal patterns relevant to the video modality. The mechanism maintains $O(N)$ linear complexity, enabling efficient temporal cross-modal feature extraction.}
    \label{fig:complementary_temporal_attention}
\end{figure}

While spatial attention captures where cross-modal interactions occur, temporal dynamics are equally critical in audio-visual learning. Audio and visual events unfold over time with complex synchronization patterns—speech articulation aligns with lip movements, sound onsets coincide with visual actions. Our Complementary Temporal Attention pathway exploits these temporal dependencies by identifying when features in one modality provide complementary information to the other, as shown in \cref{fig:complementary_temporal_attention}.

To extract temporal complementarity, we operate along the time dimension by permuting the flattened inputs $\mathbf{V}', \mathbf{A}' \in \{0, 1\}^{T \times C \times N}$ to $N \times C \times T$, treating time as the sequence dimension. We then compute asymmetric temporal projections:
\begin{equation}
    \mathbf{Q}_v^{(t)} = \text{SN}_Q(\text{BN}(\text{Conv1D}(\mathbf{V}'_{\text{perm}}, \mathbf{W}_Q^{v,t}))), \quad \mathbf{K}_a^{(t)} = \text{SN}_K(\text{BN}(\text{Conv1D}(\mathbf{A}'_{\text{perm}}, \mathbf{W}_K^{a,t}))),
\end{equation}
where $\mathbf{Q}_v^{(t)}, \mathbf{K}_a^{(t)} \in \{0, 1\}^{N \times C \times T}$ are then permuted back to $T \times C \times N$ for consistency. This formulation enables the network to learn which temporal patterns in the audio stream are relevant to the temporal evolution of visual content.

We compute the temporal attention mask through channel aggregation, analogous to the spatial pathway (see \cref{fig:complementary_temporal_attention}):
\begin{equation}
    \mathbf{A}_t^{(t)} = \text{SN}\left(\sum_{c=1}^{C} \mathbf{Q}_{v}^{(t)}[t, c, :]\right), \quad \mathbf{A}_t^{(t)} \in \{0, 1\}^{T \times 1 \times N},
\end{equation}
yielding per-timestep binary masks that identify complementary temporal patterns between modalities. The complementary temporal features are then extracted via selective masking:
\begin{equation}
    \mathbf{T}^{v \leftarrow a} = \mathbf{A}_t^{(t)} \odot \mathbf{K}_a^{(t)},
\end{equation}
where $\mathbf{T}^{v \leftarrow a} \in \{0, 1\}^{T \times C \times N}$ captures temporal dependencies between audio and visual streams. As with spatial features, we apply a spiking \ac{MLP} with residual connection for feature refinement:
\begin{equation}
    \mathbf{T}_{\text{out}}^{v \leftarrow a} = \mathbf{T}^{v \leftarrow a} + \text{MLP}(\mathbf{T}^{v \leftarrow a}),
\end{equation}
enabling nonlinear transformation while maintaining spike-form processing throughout the pathway.

\subsubsection*{Cross-Modal Feature Fusion and Residual Integration}
\begin{figure}[th]
    \centering
    \includegraphics[width=\textwidth]{imgs/cmqka.pdf}
    \caption{Fusion and residual integration within the \ac{CMQKA} module. The MLP-refined complementary spatial features $\mathbf{S}_{\text{out}}^{v \leftarrow a}$ and temporal features $\mathbf{T}_{\text{out}}^{v \leftarrow a}$ are pooled along their respective dimensions to produce reduced representations $\mathbf{S}_{\text{red}}^{v \leftarrow a}$ and $\mathbf{T}_{\text{red}}^{v \leftarrow a}$. Element-wise multiplication combines these reduced features into joint spatiotemporal complementary features $\mathbf{H}^{v \leftarrow a}$. A learnable residual connection integrates these cross-modal features into the original video representation $\mathbf{V}$, yielding enriched output features $\tilde{\mathbf{V}}$. A spiking MLP with residual connection further refines the fused features to produce the final output $\mathbf{V}_{\text{out}}$. This fusion strategy preserves modality-specific characteristics while enhancing representations with cross-modal complementary information.}
    \label{fig:cmqka_fusion}
\end{figure}

Having extracted complementary features along both spatial and temporal dimensions, we now address a critical design question: how should these two pathways be combined to form a unified cross-modal representation? Naive concatenation or summation would fail to model the interaction between spatial and temporal complementarity. Instead, we propose a multiplicative fusion strategy that captures the joint spatiotemporal relevance of cross-modal features, as depicted in \cref{fig:cmqka_fusion}.

We first apply dimension-specific pooling to compress each pathway's output (see \cref{fig:cmqka_fusion}). Spatial complementary features $\mathbf{S}_{\text{out}}^{v \leftarrow a}$ are averaged over spatial dimensions to yield $\mathbf{S}_{\text{red}}^{v \leftarrow a} \in \{0, 1\}^{T \times C \times 1 \times 1}$, retaining temporal and channel information while abstracting over space. Conversely, temporal complementary features $\mathbf{T}_{\text{out}}^{v \leftarrow a}$ are averaged over time to obtain $\mathbf{T}_{\text{red}}^{v \leftarrow a} \in \{0, 1\}^{1 \times C \times H \times W}$, preserving spatial structure while aggregating temporal patterns. We then fuse these reduced representations through element-wise multiplication:
\begin{equation}
    \mathbf{H}^{v \leftarrow a} = \mathbf{S}_{\text{red}}^{v \leftarrow a} \odot \mathbf{T}_{\text{red}}^{v \leftarrow a},
\end{equation}
where broadcasting produces $\mathbf{H}^{v \leftarrow a} \in \{0, 1\}^{T \times C \times H \times W}$. This multiplicative fusion ensures that only features exhibiting both spatial and temporal complementarity receive high activation, creating a joint spatiotemporal cross-modal representation.

A critical challenge in multimodal fusion is balancing modality-specific features with cross-modal complementary information. Aggressive fusion can dilute discriminative modality-specific patterns, while insufficient integration fails to leverage cross-modal synergy. Following the residual learning paradigm established by SCMRL~\cite{he_2025_enhancing_audio_visual}, we integrate cross-modal features through a learnable residual connection:
\begin{equation}
    \tilde{\mathbf{V}} = \mathbf{V} + \alpha \cdot \mathbf{H}^{v \leftarrow a},
\end{equation}
where $\alpha$ is a learnable scalar initialized to 0.25. This formulation preserves the original modality-specific features $\mathbf{V}$ while adding cross-modal complementary information $\mathbf{H}^{v \leftarrow a}$ as a residual term. The learnable parameter $\alpha$ enables the network to adaptively determine the optimal balance between unimodal and cross-modal representations based on task requirements and data characteristics.

To further enhance representational capacity, we apply a final spiking \ac{MLP} with residual connection: $\mathbf{V}_{\text{out}} = \tilde{\mathbf{V}} + \text{MLP}(\tilde{\mathbf{V}})$, enabling nonlinear feature transformation while maintaining spike-form processing throughout.

By operating bidirectionally—computing both $\mathbf{H}^{v \leftarrow a}$ for the video pathway and $\mathbf{H}^{a \leftarrow v}$ for the audio pathway—the \ac{CMQKA} module ensures symmetric information flow between modalities. Each modality benefits equally from cross-modal complementarity while maintaining linear computational complexity of $O(N)$, a critical property that enables the construction of deep hierarchical architectures infeasible with quadratic-complexity attention mechanisms.

\subsection{Deep Hierarchical Multimodal Spiking Transformer}


While the \ac{CMQKA} module provides efficient cross-modal feature extraction, achieving state-of-the-art performance on complex audio-visual tasks requires the ability to capture features at multiple spatial and temporal scales. Hierarchical architectures have proven essential in both \ac{ANN}-based vision models~\cite{he_2016_deep_residual_learning, liu_2021_swin_transformer_hierarchical} and unimodal spiking networks~\cite{zhou_2024_qkformer_hierarchical_spiking}, as they enable progressive semantic abstraction through multi-scale feature representations. However, constructing hierarchical multimodal \acp{SNN} has been fundamentally constrained by the quadratic complexity of traditional \ac{SSA}, which scales as $O(N^2)$ with respect to the number of tokens. This quadratic bottleneck makes it computationally prohibitive to process high-resolution inputs across multiple stages with progressively decreasing spatial dimensions.

The linear $O(N)$ complexity of our \ac{CMQKA} mechanism fundamentally eliminates this barrier, enabling—for the first time—the construction of deep hierarchical spiking transformers for multimodal learning. Building upon this foundation, we propose SNNergy, a three-stage hierarchical architecture that processes audio and visual modalities through separate but interacting pathways. Each stage combines spatial downsampling with cross-modal attention, enabling the network to extract features at progressively coarser spatial scales while increasing channel capacity and semantic abstraction. This hierarchical design mirrors the success of multi-scale processing in state-of-the-art vision models while maintaining the energy efficiency and temporal dynamics inherent to spike-based computation.

\subsubsection*{Architecture Overview}

SNNergy adopts a three-stage hierarchical design that processes audio and visual inputs through separate but interacting pathways. Given video input $\mathbf{X}^v \in \mathbb{R}^{T_v \times H \times W \times 3}$ and audio mel-spectrogram input $\mathbf{X}^a \in \mathbb{R}^{T_a \times H_a \times W_a \times 1}$, both modalities are first converted to spike-form representations and then processed through three stages with progressively increasing channel dimensions $\{C_1, C_2, C_3\} = \{192, 384, 768\}$ where $C_{i+1} = 2C_i$, and decreasing spatial resolutions. Each stage consists of two components: (1) a \ac{SPDS} module that performs spatial downsampling while increasing channel capacity, and (2) a stack of $D_i$ cross-modal attention blocks that enable interaction between modalities.

Formally, the architecture can be described as follows. In Stage 1 (early features), the inputs are first processed through separate SPDS stem modules that reduce spatial resolution by a factor of 4:
\begin{equation}
    \mathbf{V}^{(1)} = \text{SPDS}_v(\mathbf{X}^v), \quad \mathbf{A}^{(1)} = \text{SPDS}_a(\mathbf{X}^a),
\end{equation}
where $\mathbf{V}^{(1)}, \mathbf{A}^{(1)} \in \{0,1\}^{T \times B \times C_1 \times H/4 \times W/4}$ represent the early-stage spike features. These features are then processed through $D_1$ stacked \ac{CMQKA} blocks with bidirectional cross-modal attention:
\begin{equation}
    \mathbf{V}^{(1)}_i, \mathbf{A}^{(1)}_i = \text{CMQKA}_i(\mathbf{V}^{(1)}_{i-1}, \mathbf{A}^{(1)}_{i-1}), \quad i = 1, \ldots, D_1,
\end{equation}
where $\mathbf{V}^{(1)}_0 = \mathbf{V}^{(1)}$ and $\mathbf{A}^{(1)}_0 = \mathbf{A}^{(1)}$. Each \ac{CMQKA} block updates both modality features simultaneously through symmetric cross-modal attention as described in the previous subsection.

Stage 2 (middle features) begins with spatial downsampling through separate SPDS modules:
\begin{equation}
    \mathbf{V}^{(2)} = \text{SPDS}_v^{(2)}(\mathbf{V}^{(1)}_{D_1}), \quad \mathbf{A}^{(2)} = \text{SPDS}_a^{(2)}(\mathbf{A}^{(1)}_{D_1}),
\end{equation}
where $\mathbf{V}^{(2)}, \mathbf{A}^{(2)} \in \{0,1\}^{T \times B \times C_2 \times H/8 \times W/8}$ have doubled channel capacity and halved spatial resolution. These middle-stage features are refined through $D_2$ \ac{CMQKA} blocks:
\begin{equation}
    \mathbf{V}^{(2)}_i, \mathbf{A}^{(2)}_i = \text{CMQKA}_i^{(2)}(\mathbf{V}^{(2)}_{i-1}, \mathbf{A}^{(2)}_{i-1}), \quad i = 1, \ldots, D_2.
\end{equation}

Stage 3 (high-level features) performs final downsampling to the coarsest spatial resolution:
\begin{equation}
    \mathbf{V}^{(3)} = \text{SPDS}_v^{(3)}(\mathbf{V}^{(2)}_{D_2}), \quad \mathbf{A}^{(3)} = \text{SPDS}_a^{(3)}(\mathbf{A}^{(2)}_{D_2}),
\end{equation}
where $\mathbf{V}^{(3)}, \mathbf{A}^{(3)} \in \{0,1\}^{T \times B \times C_3 \times H/16 \times W/16}$ represent high-level semantic features. At this stage, with the spatial resolution significantly reduced, we employ $D_3$ cross-modal \ac{SSA} blocks to capture global spatiotemporal dependencies:
\begin{equation}
    \mathbf{V}^{(3)}_i, \mathbf{A}^{(3)}_i = \text{SSA-CM}_i(\mathbf{V}^{(3)}_{i-1}, \mathbf{A}^{(3)}_{i-1}), \quad i = 1, \ldots, D_3,
\end{equation}
where SSA-CM denotes cross-modal spiking self-attention. The use of quadratic-complexity \ac{SSA} is feasible at this final stage due to the dramatically reduced token count $N_3 = (H/16) \times (W/16) \ll N_1$, enabling the network to capture fine-grained global dependencies without computational overhead.

Finally, the modality-specific features are aggregated through global average pooling over spatial dimensions followed by temporal averaging:
\begin{equation}
    \mathbf{f}_v = \frac{1}{T}\sum_{t=1}^{T} \text{GAP}(\mathbf{V}^{(3)}_{D_3}[t]), \quad \mathbf{f}_a = \frac{1}{T}\sum_{t=1}^{T} \text{GAP}(\mathbf{A}^{(3)}_{D_3}[t]),
\end{equation}
where $\mathbf{f}_v, \mathbf{f}_a \in \mathbb{R}^{B \times C_3}$ represent the final feature vectors for each modality. These features are fused through concatenation or averaging to obtain the final multimodal representation $\mathbf{f} = [\mathbf{f}_v; \mathbf{f}_a]$ or $\mathbf{f} = 0.5(\mathbf{f}_v + \mathbf{f}_a)$, which is then passed through a linear classification head to produce class predictions.

\subsubsection*{Spiking Patch Downsampling with Shortcut (SPDS)}

Spatial downsampling is critical in hierarchical architectures for reducing computational cost and expanding the receptive field. However, naive downsampling in \acp{SNN} can lead to information loss and gradient degradation during training, particularly in deep networks. While inspired by the \ac{SPDS} module from QKFormer~\cite{zhou_2024_qkformer_hierarchical_spiking}, our implementation incorporates crucial architectural refinements for multimodal fusion that are not trivial adaptations. The key insight is the strategic placement of max-pooling operations \textit{before} spiking neurons rather than after, which preserves high-frequency spatial information that would otherwise be lost through spike binarization.

The \ac{SPDS} module reduces spatial resolution by a factor of 4 ($H \times W \rightarrow H/4 \times W/4$) while increasing the channel dimension from $C_{\text{in}}$ to $C_{\text{out}} = 2C_{\text{in}}$, implemented through two parallel pathways. The main pathway performs progressive downsampling through a carefully ordered sequence of operations:
\begin{equation}
    \begin{aligned}
        \mathbf{Z}_1             & = \text{MaxPool}(\text{BN}(\text{Conv}_{3\times3}(\mathbf{X}_{\text{in}}, C_{\text{in}}/2))), \\
        \mathbf{X}_1             & = \text{LIF}(\mathbf{Z}_1),                                                                   \\
        \mathbf{Z}_2             & = \text{MaxPool}(\text{BN}(\text{Conv}_{3\times3}(\mathbf{X}_1, C_{\text{out}}))),            \\
        \mathbf{X}_2             & = \text{LIF}(\mathbf{Z}_2),                                                                   \\
        \mathbf{X}_{\text{main}} & = \text{LIF}(\text{BN}(\text{Conv}_{3\times3}(\mathbf{X}_2, C_{\text{out}}))),
    \end{aligned}
\end{equation}
where $\mathbf{Z}_i$ represents the continuous-valued feature maps after max-pooling but before spiking activation. This ordering is critical: max-pooling operates on continuous activations from batch normalization, selecting the maximum response within each $3\times 3$ spatial neighborhood before the LIF neuron converts these continuous values to binary spikes. By performing spatial pooling in the continuous domain, the module captures high-frequency spatial details and local intensity variations that would be irretrievably lost if pooling operated on already-binarized spike tensors. This design preserves fine-grained spatial structure essential for multimodal alignment, where precise localization of audio-visual features is crucial for effective cross-modal fusion.

The shortcut pathway provides a direct connection through a single strided convolution:
\begin{equation}
    \mathbf{X}_{\text{shortcut}} = \text{LIF}(\text{BN}(\text{Conv}_{1\times1, s=2}(\mathbf{X}_1, C_{\text{out}}))),
\end{equation}
where the $1\times 1$ convolution with stride 2 matches the spatial and channel dimensions of the main pathway. The final output combines both pathways through element-wise addition:
\begin{equation}
    \mathbf{X}_{\text{out}} = \mathbf{X}_{\text{main}} + \mathbf{X}_{\text{shortcut}},
\end{equation}
where $\mathbf{X}_{\text{out}} \in \{0,1\}^{T \times B \times C_{\text{out}} \times H/4 \times W/4}$.

The residual connection in \ac{SPDS} serves multiple purposes. First, it provides an alternative gradient path during backpropagation, mitigating the vanishing gradient problem that commonly affects deep spiking networks~\cite{he_2016_deep_residual_learning}. Second, it preserves spike information across downsampling operations, ensuring that critical temporal patterns are not lost during spatial reduction. Third, it enables the training of deeper hierarchical architectures by facilitating information flow across stages. The combination of continuous-domain max-pooling, progressive downsampling, and residual learning makes \ac{SPDS} particularly well-suited for hierarchical multimodal spiking transformers, where maintaining both high-frequency spatial details and efficient information transmission is essential for accurate cross-modal feature alignment.


==> 05_experiment_and_results_section.tex <==
\section{Experiment}
\label{sec:experiment}

\subsection{Performance Comparison Across All Datasets}
\label{subsec:performance_comparison}

\textbf{Baselines.} We compare SNNergy against two categories of baselines: (1) \textit{ANN-based multimodal fusion methods} including OGM-EG~\cite{peng_2022_balanced_multimodal_learning} and PMR~\cite{fan_2023_pmr_prototypical_modal} with four fusion strategies each (sum, concatenation, FiLM, gated), representing conventional non-spiking approaches; and (2) \textit{SNN-based multimodal methods} including WeightAttention~\cite{liu_2022_event_based_multimodal}, SCA (Spiking Cross-modal Attention)~\cite{guo_2024_transformer_based_spiking}, CMCI (Cross-Modal Complementary Information)~\cite{zhou_2024_enhancing_snn_based}, S-CMRL (Spiking Cross-Modal Residual Learning)~\cite{he_2025_enhancing_audio_visual}, MISNET~\cite{liu_2025_towards_energy_efficient}, and TAAF-SNNs (Temporal Attention-guided Adaptive Fusion)~\cite{shen_2025_spiking_neural_networks}, which employ cross-modal attention in spiking networks but with quadratic complexity. For TAAF-SNNs, we report the performance values published in their paper~\cite{shen_2025_spiking_neural_networks} as we did not re-implement their method on our experimental setup. This comparison highlights SNNergy's advantage in achieving energy-efficient multimodal fusion with linear computational complexity through the novel \ac{CMQKA} mechanism.

\Cref{tab:performance_comparison} presents the comprehensive performance comparison of SNNergy against both ANN-based and SNN-based multimodal fusion baselines across all three benchmark datasets.

\begin{table}[htbp]
    \centering
    \caption{Performance comparison on CREMA-D, AVE, and UrbanSound8K-AV datasets. SNNergy achieves state-of-the-art results among SNN-based methods across all benchmarks. $^\dagger$ indicates reported results from the respective paper.}
    \label{tab:performance_comparison}
    \small
    \begin{tabular}{ p{0.15\textwidth} p{0.1\textwidth} p{0.2\textwidth} p{0.1\textwidth} p{0.15\textwidth}}
        \hline
        \textbf{Dataset}          & \textbf{Model}       & \textbf{Method}                                                       & \textbf{Fusion} & \textbf{Accuracy (\%)} \\
        \hline
        \multirow{17}{*}{CREMA-D} & \multirow{8}{*}{ANN} & \multirow{4}{*}{OGM-EG~\cite{peng_2022_balanced_multimodal_learning}} & SUM             & 74.80                  \\
                                  &                      &                                                                       & Concat          & 74.02                  \\
                                  &                      &                                                                       & Film            & 76.46                  \\
                                  &                      &                                                                       & Gated           & 72.67                  \\
        \cline{3-5}
                                  &                      & \multirow{4}{*}{PMR~\cite{fan_2023_pmr_prototypical_modal}}           & SUM             & 74.88                  \\
                                  &                      &                                                                       & Concat          & 69.51                  \\
                                  &                      &                                                                       & Film            & 75.73                  \\
                                  &                      &                                                                       & Gated           & 70.73                  \\
        \cline{2-5}
                                  & \multirow{9}{*}{SNN} & WeightAttention~\cite{liu_2022_event_based_multimodal}                & ---             & 70.12                  \\
        \cline{3-5}
                                  &                      & SCA~\cite{guo_2024_transformer_based_spiking}                         & ---             & 67.80                  \\
        \cline{3-5}
                                  &                      & CMCI~\cite{zhou_2024_enhancing_snn_based}                             & ---             & 71.59                  \\
        \cline{3-5}
                                  &                      & S-CMRL~\cite{he_2025_enhancing_audio_visual}                          & ---             & 71.59                  \\
        \cline{3-5}
                                  &                      & MISNET-L~\cite{liu_2025_towards_energy_efficient}                     & ---             & 75.22                  \\

                                  &                      & MISNET-XL~\cite{liu_2025_towards_energy_efficient}                    & ---             & 77.14                  \\
        \cline{3-5}
                                  &                      & TAAF-SNNs$^\dagger$~\cite{shen_2025_spiking_neural_networks}          & Concat          & 77.55                  \\
                                  &                      & TAAF-SNNs$^\dagger$~\cite{shen_2025_spiking_neural_networks}          & Sum             & 76.75                  \\
        \cline{3-5}
                                  &                      & \bf{SNNergy (ours)}                                                   & ---             & \bf{78.38}             \\
        \hline
        \multirow{17}{*}{AVE}     & \multirow{8}{*}{ANN} & \multirow{4}{*}{OGM-EG~\cite{peng_2022_balanced_multimodal_learning}} & SUM             & 62.68                  \\
                                  &                      &                                                                       & Concat          & 64.42                  \\
                                  &                      &                                                                       & Film            & 61.44                  \\
                                  &                      &                                                                       & Gated           & 64.67                  \\
        \cline{3-5}
                                  &                      & \multirow{4}{*}{PMR~\cite{fan_2023_pmr_prototypical_modal}}           & SUM             & 63.43                  \\
                                  &                      &                                                                       & Concat          & 62.69                  \\
                                  &                      &                                                                       & Film            & 61.69                  \\
                                  &                      &                                                                       & Gated           & 48.26                  \\
        \cline{2-5}
                                  & \multirow{9}{*}{SNN} & WeightAttention~\cite{liu_2022_event_based_multimodal}                & ---             & 65.92                  \\
        \cline{3-5}
                                  &                      & SCA~\cite{guo_2024_transformer_based_spiking}                         & ---             & 60.20                  \\
        \cline{3-5}
                                  &                      & CMCI~\cite{zhou_2024_enhancing_snn_based}                             & ---             & 67.91                  \\
        \cline{3-5}
                                  &                      & S-CMRL~\cite{he_2025_enhancing_audio_visual}                          & ---             & 68.15                  \\
        \cline{3-5}
                                  &                      & MISNET-L~\cite{liu_2025_towards_energy_efficient}                     & ---             & 67.24                  \\
                                  &                      & MISNET-XL~\cite{liu_2025_towards_energy_efficient}                    & ---             & 68.04                  \\
        \cline{3-5}
                                  &                      & TAAF-SNNs$^\dagger$~\cite{shen_2025_spiking_neural_networks}          & Concat          & 70.65                  \\
                                  &                      & TAAF-SNNs$^\dagger$~\cite{shen_2025_spiking_neural_networks}          & Sum             & 68.91                  \\
        \cline{3-5}
                                  &                      & \bf{SNNergy (ours)}                                                   & ---             & \bf{72.14}             \\
        \hline
        \multirow{15}{*}{Us8k-AV} & \multirow{8}{*}{ANN} & \multirow{4}{*}{OGM-EG~\cite{peng_2022_balanced_multimodal_learning}} & SUM             & 98.97                  \\
                                  &                      &                                                                       & Concat          & 98.97                  \\
                                  &                      &                                                                       & Film            & 98.74                  \\
                                  &                      &                                                                       & Gated           & 99.08                  \\
        \cline{3-5}
                                  &                      & \multirow{4}{*}{PMR~\cite{fan_2023_pmr_prototypical_modal}}           & SUM             & 99.77                  \\
                                  &                      &                                                                       & Concat          & 99.66                  \\
                                  &                      &                                                                       & Film            & 99.66                  \\
                                  &                      &                                                                       & Gated           & 99.77                  \\
        \cline{2-5}
                                  & \multirow{7}{*}{SNN} & WeightAttention~\cite{liu_2022_event_based_multimodal}                & ---             & 98.17                  \\
        \cline{3-5}
                                  &                      & SCA~\cite{guo_2024_transformer_based_spiking}                         & ---             & 97.83                  \\
        \cline{3-5}
                                  &                      & CMCI~\cite{zhou_2024_enhancing_snn_based}                             & ---             & 98.28                  \\
        \cline{3-5}
                                  &                      & S-CMRL~\cite{he_2025_enhancing_audio_visual}                          & ---             & 98.05                  \\
        \cline{3-5}
                                  &                      & MISNET-L~\cite{liu_2025_towards_energy_efficient}                     & ---             & 95.23                  \\
                                  &                      & MISNET-XL~\cite{liu_2025_towards_energy_efficient}                    & ---             & 97.12                  \\
        \cline{3-5}
                                  &                      & \bf{SNNergy (ours)}                                                   & ---             & \bf{98.74}             \\
        \hline
    \end{tabular}

\end{table}

\textbf{Overall Analysis.} Across all three benchmark datasets, SNNergy demonstrates consistent state-of-the-art performance among \ac{SNN}-based multimodal fusion methods, validating the effectiveness of our linear-complexity \ac{CMQKA} mechanism for hierarchical cross-modal feature integration. Several key trends emerge from the comprehensive evaluation. First, SNNergy achieves the largest performance gains on challenging tasks requiring subtle multimodal fusion: CREMA-D emotion recognition (+0.83\% over previous best \ac{SNN} method TAAF-SNNs) and AVE event classification (+1.49\% over TAAF-SNNs), while maintaining competitive performance on the less challenging UrbanSound8K-AV dataset. This demonstrates that our hierarchical multi-scale fusion architecture particularly benefits tasks requiring fine-grained extraction of complementary cross-modal information. Second, compared to \ac{ANN}-based baselines, SNNergy surpasses the best conventional fusion methods on CREMA-D (78.38\% vs. 76.46\% for OGM-EG with FiLM) and AVE (72.14\% vs. 64.67\% for OGM-EG with Gated), establishing that energy-efficient spiking-based multimodal fusion can exceed the accuracy of conventional continuous-valued approaches while providing substantial energy savings through event-driven computation. Third, the performance advantage of SNNergy over quadratic-complexity cross-modal attention methods (S-CMRL with \ac{CCSSA}) validates our core hypothesis: linear-complexity \ac{CMQKA} enables hierarchical multi-scale fusion that captures richer cross-modal representations than single-scale, quadratic-complexity approaches. The combination of computational efficiency and fusion effectiveness positions SNNergy as a practical solution for deploying sophisticated audio-visual intelligence in resource-constrained environments where both accuracy and energy efficiency are critical.

\subsection{Results on the AVE Dataset}
\label{subsec:results_ave}

\textbf{Dataset.} The AVE (Audio-Visual Event) dataset~\cite{tian_2018_audio_visual_event_localization} consists of 4,143 videos covering 28 event categories including human activities, animal sounds, musical instruments, and environmental sounds. While originally designed for temporal event localization, we adapt AVE for audio-visual event classification, where the goal is to predict the event category from the multimodal input. The official split allocates 3,339 videos for training with remaining samples equally divided into validation and test sets. All inputs use $128 \times 128$ spatial resolution for both visual frames and mel-spectrograms, with $T=6$ timesteps for temporal encoding.

\textbf{Results.} As shown in \Cref{tab:performance_comparison}, SNNergy achieves 72.14\% accuracy on the AVE dataset, establishing new state-of-the-art performance among \ac{SNN}-based multimodal fusion methods. This represents a significant improvement of 1.49\% over TAAF-SNNs (70.65\%), 3.99\% over S-CMRL (68.15\%), and 4.10\% over MISNET-XL (68.04\%). The performance gap is even more substantial when compared to other spiking attention mechanisms: SNNergy outperforms SCA by 11.94\% and WeightAttention by 6.22\%, demonstrating the effectiveness of our \ac{CMQKA} mechanism for cross-modal feature integration in event-driven architectures.

When compared to \ac{ANN}-based fusion methods, SNNergy significantly outperforms all baselines while maintaining the energy efficiency advantages of spiking computation. SNNergy surpasses the best \ac{ANN} baseline (OGM-EG with Gated fusion at 64.67\%) by 7.47\%, demonstrating that energy-efficient spiking-based multimodal fusion can substantially exceed the accuracy of conventional continuous-valued approaches. The AVE dataset's diverse event categories spanning human activities, animal sounds, musical instruments, and environmental sounds require robust multimodal fusion to capture cross-modal semantic relationships. SNNergy's hierarchical architecture with \ac{CMQKA} at multiple scales proves particularly effective for this event classification task, as it enables progressive extraction of complementary audio-visual features from low-level acoustic-visual patterns to high-level semantic event representations.

\subsection{Results on the CREMA-D Dataset}
\label{subsec:results_cremad}

\textbf{Dataset.} CREMA-D~\cite{cao_2014_crema_d_crowd_sourced} is a multimodal emotion recognition benchmark containing 7,442 audio-visual clips from 91 actors expressing six emotions (anger, disgust, fear, happiness, neutral, sadness). We adopt the subject-disjoint split protocol to prevent identity overfitting. All inputs use $128 \times 128$ spatial resolution for both visual frames and mel-spectrograms, with $T=6$ timesteps for temporal encoding.

\textbf{Results.} As shown in \Cref{tab:performance_comparison}, SNNergy achieves 78.38\% accuracy on the CREMA-D dataset, establishing a new state-of-the-art result among all \ac{SNN}-based multimodal fusion methods. This represents an improvement of 0.83\% over the previous best \ac{SNN} method TAAF-SNNs with concatenation fusion (77.55\%), and significant gains of 1.24\% over MISNET-XL (77.14\%), 3.16\% over MISNET-L (75.22\%), 6.79\% over S-CMRL (71.59\%), and 8.26\% over WeightAttention (70.12\%). Notably, SNNergy also surpasses the best \ac{ANN}-based fusion baseline (OGM-EG with FiLM fusion at 76.46\%) by 1.92\%, demonstrating that energy-efficient spiking-based multimodal fusion can achieve superior performance compared to conventional continuous-valued approaches.

\subsection{Results on the UrbanSound8K-AV Dataset}
\label{subsec:results_urbansound}

\textbf{Dataset.} UrbanSound8K-AV is a multimodal extension of the UrbanSound8K audio classification~\cite{salamon_2014_dataset_and_taxonomy}, containing 8,732 labeled sound excerpts from 10 urban sound categories including air conditioner, car horn, children playing, dog bark, drilling, engine idling, gun shot, jackhammer, siren, and street music. We pair each audio clip with synchronized video frames and apply stratified 80/10/10 train/validation/test splits to maintain class balance. All inputs use $128 \times 128$ spatial resolution for both visual frames and mel-spectrograms, with $T=6$ timesteps for temporal encoding.

\textbf{Results.} As shown in \Cref{tab:performance_comparison}, SNNergy achieves 98.74\% accuracy on the UrbanSound8K-AV dataset, demonstrating strong performance among \ac{SNN}-based multimodal fusion methods. While \ac{ANN}-based methods achieve near-perfect accuracy on this dataset (PMR with SUM/Gated fusion at 99.77\%), SNNergy maintains competitive performance with substantially lower energy consumption through sparse, event-driven spiking computation. Among \ac{SNN} baselines, SNNergy outperforms CMCI by 0.46\%, WeightAttention by 0.57\%, S-CMRL by 0.69\%, SCA by 0.91\%, and MISNET-XL by 1.62\%, establishing state-of-the-art results among energy-efficient multimodal fusion approaches.

The UrbanSound8K-AV dataset exhibits characteristics that differ significantly from AVE and CREMA-D: urban sound categories are highly distinctive with strong acoustic signatures (e.g., gun shot, siren, jackhammer), making the classification task less challenging compared to subtle emotion recognition or diverse event categorization. This explains the overall high performance across all methods. However, the dataset still benefits from multimodal fusion, as visual context provides complementary cues for sound source localization and disambiguation. For instance, distinguishing between different engine sounds (car vs. jackhammer) becomes more reliable when visual information about the sound source is incorporated. SNNergy's hierarchical \ac{CMQKA} mechanism enables effective audio-visual fusion even for highly distinctive sound categories, extracting cross-modal complementarity that enhances classification confidence.The smaller performance gap between \ac{SNN} and \ac{ANN} methods on this dataset (compared to AVE and CREMA-D) suggests that the task complexity is relatively low, with less room for improvement through sophisticated fusion mechanisms. 

\subsection{Analysis of the CMQKA Mechanism}
\label{subsec:cmqka_analysis}

In this section, we analyze the computational complexity and energy efficiency of the proposed \ac{CMQKA} mechanism, demonstrating its advantages over conventional cross-modal attention approaches.

\subsubsection*{Complexity Analysis}

We analyze the computational complexity of \ac{CMQKA} to demonstrate its linear scaling with respect to the number of tokens, in contrast to the quadratic complexity of \ac{SSA}-based approaches. Let $N = H \times W$ denote the number of spatial tokens, $C$ the channel dimension, and $T$ the number of timesteps.

\textbf{Complementary Spatial Attention.} The spatial attention pathway operates on inputs $\mathbf{V}', \mathbf{A}' \in \{0,1\}^{T \times C \times N}$. The Conv1D projections for Query and Key matrices require $O(TNC^2)$ operations each, where $\mathbf{W}_Q, \mathbf{W}_K \in \mathbb{R}^{C \times C}$. The critical distinction from \ac{SSA} occurs in the attention computation. Instead of computing the pairwise attention matrix $\mathbf{Q}\mathbf{K}^T \in \mathbb{R}^{N \times N}$, we perform channel-wise aggregation:
\begin{equation}
    \mathbf{A}_t^{(s)}[n] = \text{SN}\left(\sum_{c=1}^{C} \mathbf{Q}_v[t, c, n]\right), \quad \forall n \in \{1, \ldots, N\},
\end{equation}
producing an attention vector $\mathbf{A}_t^{(s)} \in \{0,1\}^{T \times 1 \times N}$ with complexity $O(TNC)$. The complementary features are then extracted through Hadamard masking $\mathbf{S}^{v \leftarrow a} = \mathbf{A}_t^{(s)} \odot \mathbf{K}_a$, requiring $O(TNC)$ element-wise multiplications. Post-projection and MLP operations contribute $O(TNC^2)$, yielding total spatial attention complexity $\mathcal{C}_{\text{spatial}} = O(TNC^2)$.

\textbf{Complementary Temporal Attention.} The temporal pathway follows an analogous structure, operating along the time dimension with the same complexity $\mathcal{C}_{\text{temporal}} = O(TNC^2)$.

\textbf{Fusion Operations.} Spatial and temporal pooling, multiplicative fusion, and residual integration collectively require $O(TNC)$ operations. Therefore, the total \ac{CMQKA} complexity is:
\begin{equation}
    \mathcal{C}_{\text{CMQKA}} = \mathcal{C}_{\text{spatial}} + \mathcal{C}_{\text{temporal}} + \mathcal{C}_{\text{fusion}} = O(TNC^2).
\end{equation}
Since $C$ is a fixed architectural hyperparameter independent of input resolution, the complexity is linear in the number of tokens $N$: $\mathcal{C}_{\text{CMQKA}} = O(TN)$.

\textbf{Comparison with CCSSA.} In contrast, the \ac{CCSSA} mechanism~\cite{he_2025_enhancing_audio_visual} computes the full attention matrix $\mathbf{Q}\mathbf{K}^T \in \mathbb{R}^{N \times N}$, resulting in $\mathcal{C}_{\text{CCSSA}} = O(TN^2C)$. The complexity reduction factor is:
\begin{equation}
    \frac{\mathcal{C}_{\text{CCSSA}}}{\mathcal{C}_{\text{CMQKA}}} = \frac{O(TN^2C)}{O(TNC^2)} = O\left(\frac{N}{C}\right).
\end{equation}
For typical configurations where $N \gg C$ (e.g., $N = 1024$ for $32 \times 32$ feature maps vs. $C = 192$), \ac{CMQKA} achieves significant computational savings that grow with input resolution. This efficiency enables hierarchical multimodal architectures: for a three-stage network with resolutions $\{N, N/4, N/16\}$, total complexity scales as $\approx 1.3N$ with \ac{CMQKA} versus $\approx N^2$ with \ac{CCSSA}, making multi-scale cross-modal processing computationally feasible.

\textbf{Empirical FLOPs Measurements.} To validate the theoretical complexity advantages, we conduct empirical measurements comparing computational efficiency across stages 1 and 2 of the hierarchical architecture. \Cref{fig:flops_comparison} presents the floating-point operations comparison between different architectural configurations. The results demonstrate that \ac{CMQKA}'s linear complexity translates directly into reduced computational requirements: as the spatial resolution increases from Stage 2 to Stage 1, the FLOPs gap between quadratic-complexity attention (e.g., \ac{CCSSA}) and our linear-complexity \ac{CMQKA} widens substantially. This scaling behavior validates the theoretical complexity analysis, where the reduction factor of $O(N/C)$ becomes increasingly significant at higher resolutions. The FLOPs savings are particularly pronounced in Stage 1, where finer-grained spatial tokens ($H \times W$) require more extensive attention computation.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/flops_comparison_stage1-2.pdf}
    \caption{FLOPs comparison across stages 1 and 2, demonstrating the computational efficiency advantage of \ac{CMQKA}'s linear-complexity attention mechanism. The gap between quadratic and linear attention grows with spatial resolution, validating the scalability benefits of our approach.}
    \label{fig:flops_comparison}
\end{figure}

\textbf{Runtime Performance.} \Cref{fig:runtime_comparison} presents the measured inference runtime across stages. The results show that \ac{CMQKA} achieves faster inference times compared to quadratic-complexity alternatives, with the performance advantage scaling with spatial resolution. This runtime efficiency is crucial for real-time audio-visual processing applications where low latency is required. The reduced computational complexity directly translates into faster forward pass execution, enabling SNNergy to process multimodal inputs with minimal delay. Combined with the sparse firing rates of spiking computation, the runtime savings make SNNergy practical for deployment in time-critical applications such as live video analysis, interactive robotics, and real-time surveillance systems.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/runtime_comparison_stage1-2.pdf}
    \caption{Runtime comparison across stages 1 and 2, showing the inference speed advantage of linear-complexity \ac{CMQKA}. Faster execution enables real-time multimodal processing for latency-sensitive applications.}
    \label{fig:runtime_comparison}
\end{figure}

\subsubsection*{Energy Efficiency Analysis}

Beyond computational complexity, the energy efficiency of spiking-based multimodal fusion is critical for deployment in resource-constrained environments. SNNergy achieves remarkable energy efficiency through event-driven binary spike operations, where computations occur only when spikes are present. We analyze the theoretical energy consumption following established neuromorphic hardware energy models~\cite{horowitz_2014_computing_energy_problem, zhou_2024_qkformer_hierarchical_spiking}.

\textbf{Synaptic Operations.} The fundamental unit of computation in SNNs is the \textit{Synaptic Operation} (SOP), which represents spike-based accumulate (AC) operations rather than the multiply-accumulate (MAC) operations used in ANNs. For a given layer or module $l$ in SNNergy, the number of synaptic operations is determined by the firing rate, temporal dynamics, and architectural complexity:
\begin{equation}
    \text{SOP}^l = f_r^l \times T \times \text{FLOPs}^l,
\end{equation}
where $f_r^l$ denotes the average firing rate of layer $l$ (the proportion of neurons emitting spikes), $T$ is the number of time steps, and $\text{FLOPs}^l$ represents the equivalent floating-point operations that would be required for the same computation in an ANN. The firing rate $f_r^l$ is empirically measured during inference and typically ranges from 0.05 to 0.35 across different stages of the network, reflecting the sparse event-driven nature of spiking computation.

\textbf{Hardware Energy Model.} Following prior work on neuromorphic energy estimation~\cite{horowitz_2014_computing_energy_problem, zhou_2024_qkformer_hierarchical_spiking}, we adopt the 45nm CMOS technology node as the reference hardware platform. On this substrate, multiply-accumulate operations consume $E_{\text{MAC}} = 4.6\text{ pJ}$ per operation, while spike-based accumulate operations require only $E_{\text{AC}} = 0.9\text{ pJ}$ per operation—approximately $5\times$ lower energy due to the elimination of multiplication. Batch normalization layers can be fused into preceding convolutional or linear layers during deployment through algebraic equivalence~\cite{ding_2019_acnet_strengthening_kernel, ding_2021_repvgg_making_vgg}, and thus their energy cost is subsumed into the fused operations and not counted separately.

\textbf{SNNergy Energy Consumption.} The total energy consumption of SNNergy for processing a single audio-visual sample is computed by summing the synaptic operations across all spiking layers and modules, weighted by the accumulate operation energy:
\begin{equation}
    E_{\text{SNNergy}} = E_{\text{AC}} \times \left( \sum_{i=1}^{L_{\text{conv}}} \text{SOP}_i^{\text{conv}} + \sum_{j=1}^{L_{\text{CMQKA}}} \text{SOP}_j^{\text{CMQKA}} + \sum_{k=1}^{L_{\text{SSA}}} \text{SOP}_k^{\text{SSA}} + \sum_{m=1}^{L_{\text{MLP}}} \text{SOP}_m^{\text{MLP}} \right),
\end{equation}
where $L_{\text{conv}}$, $L_{\text{CMQKA}}$, $L_{\text{SSA}}$, and $L_{\text{MLP}}$ denote the number of convolutional layers, \ac{CMQKA} modules, cross-modal \ac{SSA} modules (used only in Stage 3), and spiking MLP layers, respectively. Critically, all operations in SNNergy after the initial encoding layer operate on binary spike tensors, enabling the exclusive use of sparse accumulate operations rather than expensive multiplications.

\textbf{ANN Baseline Energy.} For comparison, the energy consumption of equivalent ANN-based multimodal fusion architectures is calculated using standard multiply-accumulate operations:
\begin{equation}
    E_{\text{ANN}} = E_{\text{MAC}} \times \text{FLOPs}_{\text{total}},
\end{equation}
where $\text{FLOPs}_{\text{total}}$ represents the total floating-point operations required for the entire forward pass through the network. Since ANNs operate on continuous-valued activations with dense computations at every timestep, they incur significantly higher energy costs compared to the sparse, event-driven processing in SNNergy.

\textbf{Energy Efficiency Gains.} The energy advantage of SNNergy arises from three synergistic factors: (i) \textit{Sparse firing rates}: typical firing rates of $f_r \approx 0.05$--$0.35$ mean that only 5--35\% of potential operations are executed, dramatically reducing computation compared to dense ANN processing; (ii) \textit{Binary spike operations}: the elimination of multiplication in favor of accumulation reduces per-operation energy by $5\times$; (iii) \textit{Linear-complexity attention}: \ac{CMQKA}'s $O(N)$ complexity versus quadratic $O(N^2)$ attention in conventional transformers reduces the number of operations, compounding energy savings across hierarchical stages. Collectively, these factors enable SNNergy to achieve multimodal fusion with substantially lower energy consumption than comparable ANN architectures while maintaining competitive recognition accuracy, as demonstrated in our experimental results.

\subsubsection*{Memory Analysis}

Memory complexity is a critical factor for deployment on resource-constrained neuromorphic hardware platforms where memory bandwidth is a primary bottleneck. The linear-complexity \ac{CMQKA} mechanism reduces memory complexity from $O(N^2)$ to $O(N)$ by maintaining only the attention vector $\mathbf{A}_t \in \{0,1\}^{N}$ rather than the full $N \times N$ attention matrix required by quadratic-complexity approaches such as \ac{CCSSA}.

\textbf{Empirical Memory Measurements.} \Cref{fig:memory_comparison} illustrates memory consumption patterns across stages 1 and 2 of the hierarchical architecture. The results demonstrate that \ac{CMQKA} maintains substantially lower memory footprint compared to quadratic-complexity attention mechanisms. This reduction becomes especially important in hierarchical architectures where multiple fusion stages operate in parallel: maintaining quadratic-complexity attention across all stages would require excessive memory allocation, limiting the feasibility of multi-scale processing. SNNergy's linear memory scaling enables efficient hierarchical fusion while remaining compatible with the memory constraints of edge deployment scenarios.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/memory_comparison_stage1-2.pdf}
    \caption{Memory consumption comparison across stages 1 and 2. \ac{CMQKA}'s $O(N)$ memory complexity versus $O(N^2)$ for quadratic attention significantly reduces memory footprint, particularly critical for neuromorphic hardware deployment.}
    \label{fig:memory_comparison}
\end{figure}

\textbf{Comprehensive Efficiency Summary.} \Cref{fig:efficiency_analysis} provides an integrated view of the efficiency achieved by \ac{CMQKA} across all measured dimensions: FLOPs, memory, and runtime. The analysis reveals that linear-complexity attention provides consistent efficiency improvements that compound across the hierarchical architecture. Importantly, these empirical measurements validate our theoretical complexity analysis: the practical benefits of $O(N)$ versus $O(N^2)$ scaling are not merely asymptotic theoretical advantages but translate into tangible computational savings even at moderate resolutions ($128 \times 128$ inputs). The efficiency gains become more pronounced in hierarchical multi-stage architectures where fusion operations are repeated at multiple scales, making \ac{CMQKA} an enabling technology for sophisticated multimodal fusion in energy-constrained environments.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/efficiency_analysis_stage1-2.pdf}
    \caption{Comprehensive efficiency analysis integrating FLOPs, memory, and runtime metrics across stages 1 and 2. The consistent efficiency advantages across all dimensions demonstrate \ac{CMQKA}'s effectiveness as a practical solution for energy-efficient hierarchical multimodal fusion.}
    \label{fig:efficiency_analysis}
\end{figure}

These efficiency measurements provide concrete evidence that SNNergy's design principles—linear-complexity attention, hierarchical multi-scale fusion, and event-driven spiking computation—collectively enable practical deployment of sophisticated audio-visual intelligence on resource-constrained platforms. The demonstrated efficiency gains in FLOPs, memory, and runtime, combined with the competitive accuracy results presented earlier, position SNNergy as a viable solution for bringing multimodal fusion capabilities to edge devices, mobile platforms, and neuromorphic processors.

\subsection{Ablation Study}
\label{subsec:ablation_study}

\subsubsection*{Temporal Encoding Depth Analysis}

\begin{table}[htbp]
    \centering
    \caption{Ablation Study: Audio-Visual Timestep Analysis on AVE and CREMA-D datasets.}
    \label{tab:ablation_timesteps}
    \begin{tabular}{llcc}
        \hline
        \textbf{Dataset} & \textbf{Timestep} & \textbf{Top-1 Accuracy (\%)} & \textbf{Test Loss} \\
        \hline
        \multirow{4}{*}{AVE} & 1                 & 64.18                        & 1.2972             \\
                             & 2                 & 68.66                        & 1.2867             \\
                             & 4                 & 69.99                        & 1.2108             \\
                             & 6                 & 72.14                        & 1.1667             \\
        \hline
        \multirow{4}{*}{CREMA-D} & 1                 & 72.63                        & 0.8299             \\
                                 & 2                 & 73.71                        & 0.7873             \\
                                 & 4                 & 75.75                        & 0.7504             \\
                                 & 6                 & 78.38                        & 0.7302             \\
        \hline
    \end{tabular}
\end{table}

To investigate the impact of temporal depth on multimodal fusion performance, we conduct an ablation study varying the number of timesteps $T \in \{1, 2, 4, 6\}$ on the AVE and CREMA-D datasets while maintaining all other architectural configurations constant. As shown in \Cref{tab:ablation_timesteps}, SNNergy exhibits consistent performance improvement as temporal resolution increases across both benchmarks. For the AVE dataset, accuracy rises from 64.18\% at $T=1$ to 72.14\% at $T=6$, representing a substantial gain of 7.96\%. A similar trend is observed on the CREMA-D dataset, where performance improves from 72.63\% to 78.38\% (+5.75\%). This consistent upward trend validates that increased temporal encoding depth enables more precise spike-timing-dependent feature representations, which are critical for capturing fine-grained cross-modal synchronization in audio-visual events and emotions.

The test loss exhibits a corresponding monotonic decrease for both datasets (AVE: 1.2972 to 1.1667; CREMA-D: 0.8299 to 0.7302), confirming improved model convergence and generalization with higher temporal resolution. Notably, the performance gain exhibits diminishing returns on both benchmarks, where the marginal utility of additional timesteps decreases beyond $T=4$. Based on this analysis, we adopt $T=6$ as the standard configuration for all subsequent experiments, balancing fusion accuracy with computational cost.

\subsubsection*{Component Contribution Analysis}
\label{sec:ablation}

\begin{table}[htbp]
\centering
\caption{Ablation study results on the AVE and CREMA-D datasets showing the contribution of spatial and temporal components.}
\label{tab:ablation}
\begin{tabular}{llcc}
        \hline
        \textbf{Dataset} & \textbf{Component} & \textbf{Top-1 Accuracy (\%)} & \textbf{Test Loss} \\
        \hline
        \multirow{3}{*}{AVE} & Spatial-only                & 63.68  & 1.3691             \\
                             & Temporal-only               & 70.15 & 1.1849             \\
                             & Spatiotemporal              & 72.14 & 1.1667            \\
        \hline
        \multirow{3}{*}{CREMA-D} & Spatial-only                & 77.78  & 0.7422             \\
                                 & Temporal-only               & 77.24 & 0.7749             \\
                                 & Spatiotemporal              & 78.38 & 0.7302               \\
        \hline
    \end{tabular}

\end{table}

To understand the contribution of different components to the overall performance of our model, we conducted an ablation study on the AVE and CREMA-D datasets. We evaluated three variants of our model: spatial-only, temporal-only, and spatiotemporal (both spatial and temporal components combined).

As shown in Table~\ref{tab:ablation}, the results vary across datasets, highlighting the different characteristics of audio-visual information in each task. For the AVE dataset, the temporal-only model (70.15\%) significantly outperforms the spatial-only model (63.68\%), indicating that temporal dynamics are more discriminative for event localization. However, for the CREMA-D dataset, the spatial-only model (77.78\%) achieves higher accuracy than the temporal-only model (77.24\%), suggesting that spatial facial expressions and visual cues are particularly strong indicators for emotion recognition.

In both cases, combining both spatial and temporal components in the spatiotemporal model yields the best performance, achieving 72.14\% on AVE and 78.38\% on CREMA-D. This consistent improvement demonstrates that spatial and temporal features provide complementary information across different audio-visual tasks. The integration of both pathways through our \ac{CMQKA} mechanism effectively captures these multifaceted relationships, leading to superior classification performance.

Table~\ref{tab:ablation} summarizes the results of our ablation study, clearly showing the incremental benefit of incorporating both spatial and temporal modalities in our architecture.




\subsubsection*{Spike Firing Rate Analysis}

\begin{table}[htbp]
    \centering
    \caption{Spike firing rates in CMQKA attention blocks across stages. Values are averaged across video/audio modalities and spatial/temporal paths. Results show attention masks (Attn) have significantly higher firing rates than Q/K neurons, indicating their role as learned gating mechanisms.}
    \label{tab:firing_rates}
    \begin{tabular}{l|ccc}
        \hline
        \textbf{Component} & \textbf{CM1 (fr)} & \textbf{CM2 (fr)} & \textbf{SSA (fr)} \\
        \hline
        \multicolumn{4}{c}{\textbf{QK Attention Blocks}}                               \\
        \hline
        Q                  & 0.1227            & 0.1420            & 0.1509            \\
        K                  & 0.1243            & 0.1371            & 0.1455            \\
        Attn               & 0.8138            & 0.7908            & 0.3094            \\
        \hline
        \multicolumn{4}{c}{\textbf{MLP Feed-Forward Blocks}}                           \\
        \hline
        Layer1             & 0.1330            & 0.1447            & 0.1330            \\
        Layer2             & 0.1309            & 0.1431            & 0.1425            \\
        \hline
    \end{tabular}
\end{table}

To understand the computational efficiency of SNNergy's hierarchical architecture, we analyze spike firing rates across different components and stages. As shown in \Cref{tab:firing_rates}, the firing rate distribution reveals several critical insights into the energy-efficient design of our \ac{CMQKA} mechanism. Query and Key neurons maintain remarkably low firing rates of approximately 12--15\% across all stages, demonstrating the sparse, event-driven nature of cross-modal attention computation. This sparsity directly translates to energy savings, as only 12--15\% of neurons actively consume power per timestep, compared to 100\% activation in conventional \ac{ANN}-based attention mechanisms.

The attention mask neurons (Attn) exhibit substantially higher firing rates ranging from 31\% to 81\%, which is 6--7$\times$ higher than Query/Key neurons. This elevated firing rate indicates that the attention masks function as active learned gating mechanisms rather than passive filtering operations. The threshold of 0.5 in the attention \ac{LIF} neurons creates a binary selection gate that adaptively determines which cross-modal tokens are relevant for fusion. Notably, the firing rates decrease hierarchically across stages: CM1 (81.38\%) $>$ CM2 (79.08\%) $>$ SSA (30.94\%). This progressive reduction suggests that early stages perform broad cross-modal feature extraction with high token selection, while later stages focus on selective refinement of discriminative multimodal features. The dramatic drop in SSA firing rate (30.94\%) reflects the coarser spatial resolution at Stage 3 ($H/16 \times W/16$), where fewer but more semantically meaningful tokens require attention.

The \ac{MLP} feed-forward blocks maintain stable firing rates of approximately 13--14\% across all stages and layers, ensuring balanced feature transformation without excessive spike activity. The consistency of MLP firing rates across Layer1 (expansion) and Layer2 (projection) indicates stable gradient flow and effective residual learning throughout the hierarchical architecture. Importantly, the similar firing rates between Query/Key neurons and MLP layers demonstrate that SNNergy achieves computational balance: cross-modal attention mechanisms do not introduce disproportionate spike activity compared to standard feed-forward processing.

From an energy efficiency perspective, these firing rate patterns validate SNNergy's design principles. The low firing rates in Query/Key projections (12--15\%) and MLP layers (13--14\%) ensure that the majority of computations remain sparse and event-driven, directly reducing synaptic operations and power consumption. The higher firing rates in attention masks (31--81\%) are justified by their critical role as adaptive gating mechanisms that enable effective cross-modal fusion. Since attention masks operate on channel-aggregated representations rather than full token-to-token matrices, their computational overhead remains manageable despite higher firing rates. The hierarchical decrease in attention firing rates further contributes to efficiency, as later stages process fewer tokens with more focused selection.

==> 06_conclusion_section.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we presented SNNergy, a novel energy-efficient multimodal fusion framework for audio-visual intelligence that addresses the fundamental challenge of efficient cross-modal feature integration in resource-constrained environments. Our key contribution is the \ac{CMQKA} mechanism, which achieves linear computational complexity for multimodal fusion through query-key attention while maintaining competitive recognition performance across diverse audio-visual tasks.

The hierarchical architecture of SNNergy progressively integrates multimodal features across three stages with increasing semantic abstraction, enabled by the \ac{SPDS} module that preserves spike information during spatial downsampling. Experimental results on CREMA-D, AVE, and UrbanSound8K-AV datasets demonstrate that SNNergy achieves superior performance compared to existing \ac{SNN}-based multimodal methods while maintaining the energy efficiency advantages of event-driven spiking computation.

Our work demonstrates that efficient multimodal fusion is achievable in spiking neural networks without sacrificing performance, opening new possibilities for deploying sophisticated audio-visual intelligence on edge devices and neuromorphic hardware. The linear complexity of \ac{CMQKA} makes SNNergy particularly suitable for real-time applications where both computational efficiency and energy constraints are critical.

Future work will explore extending SNNergy to other multimodal domains beyond audio-visual processing, investigating adaptive temporal encoding strategies to further optimize energy consumption, and deploying the framework on neuromorphic hardware platforms to validate end-to-end energy efficiency in practical scenarios.




